Characterizing Generalization under Out-Of-Distribution Shifts in Deep Metric Learning

Deep Metric Learning (DML) aims to find representations suitable for zero-shot transfer to a priori unknown test distributions. However, common evaluation protocols only test a single, fixed data split in which train and test classes are assigned randomly. More realistic evaluations should consider a broad spectrum of distribution shifts with potentially varying degree and difficulty. In this work, we systematically construct train-test splits of increasing difficulty and present the ooDML benchmark to characterize generalization under out-of-distribution shifts in DML. ooDML is designed to probe the generalization performance on much more challenging, diverse train-to-test distribution shifts. Based on our new benchmark, we conduct a thorough empirical analysis of state-of-the-art DML methods. We find that while generalization tends to consistently degrade with difficulty, some methods are better at retaining performance as the distribution shift increases. Finally, we propose few-shot DML as an efficient way to consistently improve generalization in response to unknown test shifts presented in ooDML. Code available here: https://github.com/CompVis/Characterizing_Generalization_in_DML.

==> figures/fewshot_cars.tex <==

\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{images/few_shot_compare_car_R1.png}
    \caption{\textit{Few-Shot adaptation of DML representations on CARS196 dataset.} Columns 1-4 show average recall@1 performance over 10 episodes of 2- and 5-shot adaption for various DML approaches. Columns 5-6 compares the individual few- and zero-shot results from columns 1-4.}
    \label{fig:fewshot_car_recall}
\end{figure}



==> figures/pretrained_fewshot_comp.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{images/pretrained_fewshot_generalization_comp.png}
    \caption{\textit{Comparison} of best and worst DML objectives trained with a ResNet50-backbone against different training models and networks which are NOT adapted to the training data at hand in a few-shot setting. What can be seen is that changes in pretraining method and architecture, similar to the zero-shot case, can offer additional OOD generalization benefits in a few-shot approach. Again however, training and adaptation does provide consistent generalization performance.}
    \label{fig:pretrained_fewshot_comp}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

==> tables/Full_Results.tex <==
\begin{table}[h]
\caption{\textit{Detailed Comparison of Recall@1 and NMI performances against well performing DML objectives examined in section \ref{sec:comp}.} This is the complete version to table \ref{tab:relative_results}. All results are computed over 5-run averages. ($^*$) For Margin Loss and SOP, we found $\beta=0.9$ to give better distillation results without notably influencing baseline performance.}
\resizebox{\textwidth}{!}{
 \footnotesize
   \setlength\tabcolsep{1.4pt}
   \centering
   %\begin{tabular}{l|c|ccc|c}
   \begin{tabular}{l|c|c||c|c||c|c}
     \toprule
     \multicolumn{1}{l}{\textbf{Benchmarks}$\rightarrow$} & \multicolumn{2}{c}{\textsc{CUB200-2011}} & \multicolumn{2}{c}{\textsc{CARS196}} & \multicolumn{2}{c}{\textsc{SOP}} \\
     \midrule
     \textbf{Approaches} $\downarrow$ & R@1 & NMI & R@1 & NMI & R@1 & NMI\\
    \midrule
    \textbf{Margin}($^*$) & $63.09\pm0.46$ & $68.21\pm0.33$ & $79.86\pm0.33$ & $67.36\pm0.34$ & $78.43\pm0.07$ & $90.40\pm0.03$\\        
    + DSD & $65.11\pm0.18$ & $69.65\pm0.44$ & $83.19\pm0.18$ & $69.28\pm0.56$ & $79.05\pm0.12$ & $90.52\pm0.18$\\
    + DSDA & $65.77\pm0.55$ & $69.85\pm0.25$ & $83.92\pm0.08$ & $69.95\pm0.21$ & $77.78\pm0.15$ & $90.29\pm0.08$\\
    + MSD & $66.13\pm0.34$ & $70.83\pm0.27$ & $83.63\pm0.31$ & $69.80\pm0.36$ & $79.26\pm0.15$ & $90.60\pm0.10$\\
    + MSDA & $66.14\pm0.32$ & $70.82\pm0.18$ & $84.31\pm0.12$ & $70.17\pm0.30$ & $78.04\pm0.11$ & $90.45\pm0.05$\\
    + MSDF & $67.58\pm0.32$ & $71,47\pm0.19$ & $85.55\pm0.23$ & $71.68\pm0.54$ & $79.63\pm0.14$ & $90.70\pm0.09$\\
    + MSDFA & $67.21\pm0.23$ & $71.43\pm0.25$ & $86.45\pm0.35$ & $71.46\pm0.24$ & $78.82\pm0.09$ & $90.49\pm0.06$\\
    
    \midrule
    \textbf{R-Margin} & $64.93\pm0.42$ & $68.36\pm0.32$ & $82.37\pm0.13$ & $68.66\pm0.47$ & $77.58\pm0.11$ & $90.42\pm0.03$\\ 
    + DSD & $66.58\pm0.08$ & $70.03\pm0.41$ & $84.64\pm0.16$ & $70.87\pm0.18$ & $77.86\pm0.10$ & $90.50\pm0.03$\\
    + DSDA & $67.11\pm0.43$ & $70.39\pm0.48$ & $84.32\pm0.36$ & $70.85\pm0.16$ & $77.79\pm0.11$ & $90.37\pm0.04$\\
    + MSD & $66.81\pm0.27$ & $70.47\pm0.16$ & $85.01\pm0.10$ & $71.67\pm0.40$ & $78.00\pm0.06$ & $90.47\pm0.04$\\
    + MSDA & $67.31\pm0.41$ & $71.01\pm0.24$ & $85.34\pm0.17$ & $71.85\pm0.20$ & $77.93\pm0.06$ & $90.29\pm0.08$\\
    + MSDF & $68.12\pm0.30$ & $71.80\pm0.33$ & $85.78\pm0.22$ & $72.24\pm0.31$ & $78.57\pm0.09$ & $90.58\pm0.02$\\
    + MSDFA & $68.58\pm0.26$ & $71.64\pm0.40$ & $86.81\pm0.35$ & $71.48\pm0.29$ & $78.00\pm0.11$ & $90.41\pm0.02$\\
    \midrule
    \textbf{Multisimilarity} & $62.80\pm0.70$ & $68.55\pm0.38$ & $81.68\pm0.19$ & $69.43\pm0.38$ & $77.99\pm0.09$ & $90.00\pm0.02$\\
    + DSD & $65.57\pm0.26$ & $70.08\pm0.33$ & $83.51\pm0.20$ & $70.30\pm0.05$ & $78.23\pm0.04$& $90.08\pm0.04$\\
    + DSDA & $66.60\pm0.43$ & $70.74\pm0.40$ & $84.42\pm0.28$ & $70.36\pm0.34$ & $77.92\pm0.12$ & $89.99\pm0.04$\\
    + MSD & $65.80\pm0.16$ & $70.53\pm0.01$ & $83.98\pm0.10$ & $71.34\pm0.09$ & $78.42\pm0.09$ & $90.09\pm0.03$\\
    + MSDA & $66.96\pm0.36$ & $70.77\pm0.05$ & $85.04\pm0.14$ & $71.09\pm0.23$ & $77.98\pm0.05$ & $90.02\pm0.04$\\
    + MSDF & $67.04\pm0.29$ & $71.87\pm0.19$ & $85.69\pm0.19$ & $72.77\pm0.13$ & $78.59\pm0.08$ & $90.09\pm0.06$\\
    + MSDFA & $67.68\pm0.29$ & $71.40\pm0.21$ & $85.89\pm0.15$ & $71.45\pm0.26$ & $78.07\pm0.06$ & $89.88\pm0.10$\\
         
%     \midrule
%     \textbf{ProxyAnchor} & $64.58\pm0.23$ & $68.95\pm0.24$ & $82.55\pm0.41$ & $69.49\pm0.30$ & $77.92\pm0.09$ & $90.09\pm0.06$\\    
% + DSD & $65.50\pm0.47$ & $69.97\pm0.55$ & $83.52\pm0.11$ & $70.76\pm0.17$ & $78.33\pm0.08$ & $90.24\pm0.06$\\
% + DSDA & $65.61\pm0.36$ & $69.62\pm0.54$ & $84.81\pm0.08$ & $70.11\pm0.25$ & $77.94\pm0.05$ & $90.13\pm0.06$\\
% + MSD & $65.92\pm0.28$ & $69.88\pm0.21$ & $83.99\pm0.33$ & $70.95\pm0.19$ & $78.47\pm0.03$ & $90.29\pm0.06$\\
% + MSDA & $65.83\pm0.40$ & $70.21\pm0.51$ & $84.63\pm0.16$ & $70.58\pm0.36$ & $78.01\pm0.06$ & $90.23\pm0.01$\\
% + MSDF & $66.71\pm0.12$ & $70.60\pm0.24$ & $85.20\pm0.09$ & $71.19\pm0.18$ & $78.50\pm0.04$ & $90.31\pm0.03$\\
% + MSDFA & $66.47\pm0.36$ & $70.66\pm0.17$ & $85.59\pm0.17$ & $69.77\pm0.45$ & $78.03\pm0.05$ & $90.18\pm0.03$\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:relative_results_long}
 \end{table}


% \begin{table*}[t]
%  \small
%  \rowcolors{2}{gray!8}{white}
%   \setlength\tabcolsep{1.4pt}
%   \centering
%   %\begin{tabular}{l|c|ccc|c}
%   \begin{tabular}{l|c|c||c|c||c|c}
%      \toprule
%      \multicolumn{1}{l}{Benchmarks$\rightarrow$} & \multicolumn{2}{c}{CUB200-2011} & \multicolumn{2}{c}{CARS196} & \multicolumn{2}{c}{SOP} \\
%      \midrule
%      Approaches $\downarrow$ & R@1 & NMI & R@1 & NMI & R@1 & NMI\\
%      \midrule
%     Imagenet~\cite{imagenet} & $43.77$ & $57.56$ & $36.39$ & $37.96$ & $48.65$ & $58.64$ \\
%     \midrule
%     Angular~\cite{angular} & $62.10\pm0.27$ & $67.59\pm0.26$ & $78.00\pm0.32$ & $66.48\pm0.44$ & $73.22\pm0.07$ & $89.53\pm0.01$\\
%     ArcFace~\cite{arcface} & $62.67\pm0.67$ & $67.66\pm0.38$ & $79.16\pm0.97$ & $66.99\pm1.08$ & $77.71\pm0.15$ & $90.09\pm0.03$\\
%     Contrastive~\cite{contrastive} (D) & $61.50\pm0.17$ & $66.45\pm0.27$ & $75.78\pm0.39$ & $64.04\pm0.13$ & $73.21\pm0.04$ & $89.78\pm0.02$\\
%     Margin (D, $\beta=0.6$)~\cite{margin} & $62.50\pm0.24$ & $67.02\pm0.37$ & $77.70\pm0.32$ & $65.29\pm0.32$ & $77.38\pm0.11$ & \blue{$\mathbf{90.45\pm0.03}$}\\
%     Margin (D, $\beta=1.2$)~\cite{margin} & $\mathbf{63.09\pm0.46}$ & $68.21\pm0.33$ & $79.86\pm0.33$ & $67.36\pm0.34$ & $\mathbf{78.43\pm0.07}$ & $90.40\pm0.03$\\
%     Multisimilarity~\cite{multisimilarity} & $62.80\pm0.70$ & \blue{$\mathbf{68.55\pm0.38}$} & $\mathbf{81.68\pm0.19}$ & \blue{$\mathbf{69.43\pm0.38}$} & $77.99\pm0.09$ & $90.00\pm0.02$\\
%     Npair~\cite{npairs} & $61.63\pm0.58$ & $67.64\pm0.37$ & $77.48\pm0.28$ & $66.55\pm0.19$ & $75.86\pm0.08$ & $89.79\pm0.03$\\
%     Pnca~\cite{proxynca} & $62.80\pm0.48$ & $66.93\pm0.38$ & $78.48\pm0.58$ & $65.76\pm0.22$ & $-$ & $-$\\
%     SNR (D)~\cite{signal2noise} & $62.88\pm0.18$ & $67.16\pm0.25$ & $78.69\pm0.19$ & $65.84\pm0.52$ & $77.61\pm0.34$ & $90.10\pm0.08$\\
%     Softmax~\cite{zhai2018classification} & $61.66\pm0.33$ & $66.77\pm0.36$ & $78.91\pm0.27$ & $66.35\pm0.30$ & $76.92\pm0.64$ & $89.82\pm0.15$\\
%     \midrule
%     Triplet (D)~\cite{margin} & $62.87\pm0.35$ & $67.53\pm0.14$ & $79.13\pm0.27$ & $65.90\pm0.18$ & $77.39\pm0.15$ & $90.06\pm0.02$\\
%     Triplet (R)~\cite{semihard} & $58.48\pm0.31$ & $63.84\pm0.30$ & $70.63\pm0.43$ & $61.09\pm0.27$ & $67.86\pm0.14$ & $88.35\pm0.04$\\
%     \midrule
%     R-Margin (D, $\beta=0.6$) & \blue{$\mathbf{64.93\pm0.42}$} & $68.36\pm0.32$ & \blue{$\mathbf{82.37\pm0.13}$} & $68.66\pm0.47$ & $77.58\pm0.11$ & $90.42\pm0.03$\\

%     \bottomrule
%     \end{tabular}
%     \caption{\textit{Comparison of Recall@1 and NMI performances against various objectives} averaged over 5 runs.}
%     \label{tab:relative_results}
% \vspace{-8pt}
%  \end{table*}


==> tables/Short_Full_Results.tex <==
\begin{table*}[t]
    \caption{\textit{S2SD comparison against strong baseline objectives.} All results computed over multiple seeds. \textbf{Bold} denotes best results per loss \& benchmark,  \blue{\textbf{bluebold}} marks best results per benchmark.}
 \footnotesize
   \setlength\tabcolsep{1.4pt}
   \centering
   %\begin{tabular}{l|c|ccc|c}
   \begin{tabular}{l|c|c||c|c||c|c}
     \toprule
     \multicolumn{1}{l}{\textbf{Benchmark}$\rightarrow$} & \multicolumn{2}{c}{\textsc{CUB200-2011}} & \multicolumn{2}{c}{\textsc{CARS196}} & \multicolumn{2}{c}{\textsc{SOP}} \\
     \midrule
     \textbf{Approaches} $\downarrow$ & R@1 & NMI & R@1 & NMI & R@1 & NMI\\
    \midrule
    \textbf{Margin}, $\beta=1.2$, \cite{margin} & $63.09\pm0.46$ & $68.21\pm0.33$ & $79.86\pm0.33$ & $67.36\pm0.34$ & $78.43\pm0.07$ & $90.40\pm0.03$\\        
    + DSD & $65.11\pm0.18$ & $69.65\pm0.44$ & $83.19\pm0.18$ & $69.28\pm0.56$ & $79.05\pm0.12$ & $90.52\pm0.18$\\
    + MSD & $66.13\pm0.34$ & $70.83\pm0.27$ & $83.63\pm0.31$ & $69.80\pm0.36$ & $79.26\pm0.15$ & $90.60\pm0.10$\\
    + MSDF & $\mathbf{67.58\pm0.32}$ & $\mathbf{71.47\pm0.19}$ & $85.55\pm0.23$ & $\mathbf{71.68\pm0.54}$ & \blue{$\mathbf{79.63\pm0.15}$} & \blue{$\mathbf{90.70\pm0.09}$} \\
    + MSDFA & $67.21\pm0.23$ & $71.43\pm0.25$ & $\mathbf{86.45\pm0.35}$ & $71.46\pm0.24$ & $78.82\pm0.09$ & $90.49\pm0.06$ \\
    \hline
    \textbf{R-Margin}, $\beta=0.6$, \cite{roth2020revisiting} & $64.93\pm0.42$ & $68.36\pm0.32$ & $82.37\pm0.13$ & $68.66\pm0.47$ & $77.58\pm0.11$ & $90.42\pm0.03$\\ 
    + DSD & $66.58\pm0.08$ & $70.03\pm0.41$ & $84.64\pm0.16$ & $70.87\pm0.18$ & $77.86\pm0.10$ & $90.50\pm0.03$\\
    + MSD & $66.81\pm0.27$ & $70.47\pm0.16$ & $85.01\pm0.10$ & $71.67\pm0.40$ & $78.00\pm0.06$ & $90.47\pm0.04$\\
    + MSDF & $68.12\pm0.30$ & $\mathbf{71.80\pm0.33}$ & $85.78\pm0.22$ & $\mathbf{72.24\pm0.31}$ & $\mathbf{78.57\pm0.09}$ & $\mathbf{90.58\pm0.02}$\\
    + MSDFA & $\blue{\mathbf{68.58\pm0.26}}$ & $71.64\pm0.40$ & $\blue{\mathbf{86.81\pm0.35}}$ & $71.48\pm0.29$ & $78.00\pm0.11$ & $90.41\pm0.02$\\
    \hline
    \textbf{Multisimilarity} \cite{multisimilarity} & $62.80\pm0.70$ & $68.55\pm0.38$ & $81.68\pm0.19$ & $69.43\pm0.38$ & $77.99\pm0.09$ & $90.00\pm0.02$\\
    + DSD & $65.57\pm0.26$ & $70.08\pm0.33$ & $83.51\pm0.20$ & $70.30\pm0.05$ & $78.23\pm0.04$ & $90.08\pm0.04$\\
    + MSD & $65.80\pm0.16$ & $70.6553\pm0.01$ & $83.98\pm0.10$ & $71.34\pm0.09$ & $78.42\pm0.09$ & $90.09\pm0.03$\\        
    + MSDF & $67.04\pm0.29$ & $\blue{\mathbf{71.87\pm0.19}}$ & $85.69\pm0.19$ & $\blue{\mathbf{72.77\pm0.13}}$ & $\mathbf{78.59\pm0.08}$ & $\mathbf{90.09\pm0.06}$\\
    + MSDFA & $\mathbf{67.68\pm0.29}$ & $71.40\pm0.21$ & $\mathbf{85.89\pm0.15}$ & $71.45\pm0.26$ & $78.07\pm0.06$ & $89.88\pm0.10$ \\
         
    % \hline
    % \textbf{ProxyAnchor} \cite{kim2020proxy} & $64.58\pm0.23$ & $68.95\pm0.24$ & $82.55\pm0.41$ & $69.49\pm0.30$ & $77.92\pm0.09$ & $90.09\pm0.06$\\    
    % + DSD    & $65.50\pm0.47$ & $69.97\pm0.55$ & $83.52\pm0.11$ & $70.76\pm0.17$ & $78.33\pm0.08$ & $90.24\pm0.06$\\
    % + MSDF & $\mathbf{66.71\pm0.12}$ & $70.60\pm0.24$ & $85.20\pm0.09$ & $\mathbf{71.19\pm0.18}$ & $\mathbf{78.50\pm0.04}$ & $\mathbf{90.31\pm0.03}$\\
    % + MSDFA & $66.47\pm0.36$ & $\mathbf{70.66\pm0.17}$ & $\mathbf{85.59\pm0.17}$ & $69.77\pm0.45$ & $78.03\pm0.05$ & $90.18\pm0.03$\\
    \bottomrule
    \end{tabular}
    \label{tab:relative_results}
 \end{table*}




==> tables/Short_Full_Results_arxiv.tex <==
\begin{table*}[t]
    \caption{\textit{S2SD comparison against strong baseline objectives.} All results computed over multiple seeds. \textbf{Bold} denotes best results per loss \& benchmark,  \blue{\textbf{bluebold}} marks best results per benchmark.}
 \footnotesize
   \setlength\tabcolsep{1.4pt}
   \centering
   %\begin{tabular}{l|c|ccc|c}
   \resizebox{\textwidth}{!}{
   \begin{tabular}{l|c|c||c|c||c|c}
     \toprule
     \multicolumn{1}{l}{\textbf{Benchmark}$\rightarrow$} & \multicolumn{2}{c}{\textsc{CUB200-2011}} & \multicolumn{2}{c}{\textsc{CARS196}} & \multicolumn{2}{c}{\textsc{SOP}} \\
     \midrule
     \textbf{Approaches} $\downarrow$ & R@1 & NMI & R@1 & NMI & R@1 & NMI\\
    \midrule
    \textbf{Margin}, $\beta=1.2$, \cite{margin} & $63.09\pm0.46$ & $68.21\pm0.33$ & $79.86\pm0.33$ & $67.36\pm0.34$ & $78.43\pm0.07$ & $90.40\pm0.03$\\        
    + DSD & $65.11\pm0.18$ & $69.65\pm0.44$ & $83.19\pm0.18$ & $69.28\pm0.56$ & $79.05\pm0.12$ & $90.52\pm0.18$\\
    + MSD & $66.13\pm0.34$ & $70.83\pm0.27$ & $83.63\pm0.31$ & $69.80\pm0.36$ & $79.26\pm0.15$ & $90.60\pm0.10$\\
    + MSDF & $\mathbf{67.58\pm0.32}$ & $\mathbf{71.47\pm0.19}$ & $85.55\pm0.23$ & $\mathbf{71.68\pm0.54}$ & \blue{$\mathbf{79.63\pm0.15}$} & \blue{$\mathbf{90.70\pm0.09}$} \\
    + MSDFA & $67.21\pm0.23$ & $71.43\pm0.25$ & $\mathbf{86.45\pm0.35}$ & $71.46\pm0.24$ & $78.82\pm0.09$ & $90.49\pm0.06$ \\
    \hline
    \textbf{R-Margin}, $\beta=0.6$, \cite{roth2020revisiting} & $64.93\pm0.42$ & $68.36\pm0.32$ & $82.37\pm0.13$ & $68.66\pm0.47$ & $77.58\pm0.11$ & $90.42\pm0.03$\\ 
    + DSD & $66.58\pm0.08$ & $70.03\pm0.41$ & $84.64\pm0.16$ & $70.87\pm0.18$ & $77.86\pm0.10$ & $90.50\pm0.03$\\
    + MSD & $66.81\pm0.27$ & $70.47\pm0.16$ & $85.01\pm0.10$ & $71.67\pm0.40$ & $78.00\pm0.06$ & $90.47\pm0.04$\\
    + MSDF & $68.12\pm0.30$ & $\mathbf{71.80\pm0.33}$ & $85.78\pm0.22$ & $\mathbf{72.24\pm0.31}$ & $\mathbf{78.57\pm0.09}$ & $\mathbf{90.58\pm0.02}$\\
    + MSDFA & $\blue{\mathbf{68.58\pm0.26}}$ & $71.64\pm0.40$ & $\blue{\mathbf{86.81\pm0.35}}$ & $71.48\pm0.29$ & $78.00\pm0.11$ & $90.41\pm0.02$\\
    \hline
    \textbf{Multisimilarity} \cite{multisimilarity} & $62.80\pm0.70$ & $68.55\pm0.38$ & $81.68\pm0.19$ & $69.43\pm0.38$ & $77.99\pm0.09$ & $90.00\pm0.02$\\
    + DSD & $65.57\pm0.26$ & $70.08\pm0.33$ & $83.51\pm0.20$ & $70.30\pm0.05$ & $78.23\pm0.04$ & $90.08\pm0.04$\\
    + MSD & $65.80\pm0.16$ & $70.6553\pm0.01$ & $83.98\pm0.10$ & $71.34\pm0.09$ & $78.42\pm0.09$ & $90.09\pm0.03$\\        
    + MSDF & $67.04\pm0.29$ & $\blue{\mathbf{71.87\pm0.19}}$ & $85.69\pm0.19$ & $\blue{\mathbf{72.77\pm0.13}}$ & $\mathbf{78.59\pm0.08}$ & $\mathbf{90.09\pm0.06}$\\
    + MSDFA & $\mathbf{67.68\pm0.29}$ & $71.40\pm0.21$ & $\mathbf{85.89\pm0.15}$ & $71.45\pm0.26$ & $78.07\pm0.06$ & $89.88\pm0.10$ \\
         
    % \hline
    % \textbf{ProxyAnchor} \cite{kim2020proxy} & $64.58\pm0.23$ & $68.95\pm0.24$ & $82.55\pm0.41$ & $69.49\pm0.30$ & $77.92\pm0.09$ & $90.09\pm0.06$\\    
    % + DSD    & $65.50\pm0.47$ & $69.97\pm0.55$ & $83.52\pm0.11$ & $70.76\pm0.17$ & $78.33\pm0.08$ & $90.24\pm0.06$\\
    % + MSDF & $\mathbf{66.71\pm0.12}$ & $70.60\pm0.24$ & $85.20\pm0.09$ & $\mathbf{71.19\pm0.18}$ & $\mathbf{78.50\pm0.04}$ & $\mathbf{90.31\pm0.03}$\\
    % + MSDFA & $66.47\pm0.36$ & $\mathbf{70.66\pm0.17}$ & $\mathbf{85.59\pm0.17}$ & $69.77\pm0.45$ & $78.03\pm0.05$ & $90.18\pm0.03$\\
    \bottomrule
    \end{tabular}}
    \label{tab:relative_results}
 \end{table*}



==> tables/ablations.tex <==
%  \begin{table}[h]
%  \small
%   \centering
%   \begin{tabular}{l||c|c|c|c}
%      \toprule
%      Experiment & Setting & R@1 & Setting & R@1\\
%      \midrule

% \multirow{12}{*}{Objectives} & Margin (D), B & $62.53\pm0.35$ & Multisimilarity, B & $62.70\pm0.53$\\
%  & Margin (D), DSD & $65.11\pm0.18$ & Multisimilarity, DSD & $65.57\pm0.26$\\
%  & Margin (D), DSDA & $65.77\pm0.55$ & Multisimilarity, DSDA & $66.51\pm0.17$\\
%  & Margin (D), MSD & $66.13\pm0.34$ & Multisimilarity, MSD & $65.68\pm0.12$\\
%  & Margin (D), MSDA & $66.14\pm0.32$ & Multisimilarity, MSDA & $66.96\pm0.36$\\
%  & Margin (D), MSDFA & $67.21\pm0.23$ & Multisimilarity, MSDFA & $67.68\pm0.29$\\
%  & R-Margin, B & $64.74\pm0.33$ & ProxyAnchor, B & $64.58\pm0.23$\\
%  & R-Margin, DSD & $66.58\pm0.08$ & ProxyAnchor, DSD & $65.50\pm0.47$\\
%  & R-Margin, DSDA & $67.11\pm0.43$ & ProxyAnchor, DSDA & $65.61\pm0.36$\\
%  & R-Margin, MSD & $66.70\pm0.31$ & ProxyAnchor, MSD & $65.92\pm0.28$\\
%  & R-Margin, MSDA & $67.31\pm0.41$ & ProxyAnchor, MSDA & $65.83\pm0.40$\\
%  & R-Margin, MSDFA & $68.58\pm0.26$ & ProxyAnchor, MSDFA & $66.47\pm0.36$\\

%     \bottomrule
%     \end{tabular}
%     \caption{\textit{Experiment: Self-Distillation vs Objectives - see \ref{sec:ablations}.} See fig. \ref{fig:ablations_1}A. All results are computed over 5-run averages.}
%     \label{tab:ablations_1}
%  \end{table}
 
 
 
 
 %%%%%%%
\begin{table}[h]
 \small
   \centering
    \caption{\textit{Experiment: Comparison of concurrent self-distillation against standard 2-stage distillation.} This table also shows that training without distillation (\textit{Joint}) or training in high dimension while learning a detached low-dimensional embedding layer (\textit{Concur.}) does not benefit performance notably. See fig. \ref{fig:ablations_1}A. All results are computed over 5-run averages.}   
   \begin{tabular}{l||c|c}
     \toprule
     Experiment & Setting & R@1\\
     \midrule
     \multirow{9}{*}{Distillation} & Best Teacher (d=1024) & $66.04\pm0.17$\\
     & Base Student (d=128) & $62.70\pm0.53$\\
     & Distill Student (d=128) & $63.89\pm0.14$\\
     & Concur. Student (d=128) & $63.08\pm0.42$\\
     & Joint Student (d=128) & $62.93\pm0.22$\\
     & DSD   (d=128) & $65.57\pm0.26$\\
     & DSDA  (d=128) & $66.51\pm0.18$\\
     & MSDA (d=128) & $66.96\pm0.36$\\
     & MSDFA (d=128) & $67.68\pm0.29$\\
    \bottomrule
    \end{tabular}
    \label{tab:ablations_6}
 \end{table}



%%%%%%%%%
 \begin{table}[h]
 \small
   \centering
    \caption{\textit{Experiment: Benefit of self-distillation across embedding dimensionalities.} These results go along with \ref{fig:ablations_1}B. All results are computed over 5-run averages.}   
   \begin{tabular}{l||c|c|c|c}
     \toprule
     Experiment & Setting & R@1 & Setting & R@1\\
     \midrule
\multirow{28}{*}{Embedding Dimensionality} & Base (d=16) & $48.18\pm0.54$& MSD (d=256) & $66.90\pm0.11$\\
 & Basic (d=32) & $54.54\pm0.42$& MSD (d=512) & $67.07\pm0.02$\\     
 & Basic (d=64) & $59.31\pm0.26$& MSD (d=1024) & $66.69\pm0.11$\\ 
 & Basic (d=128) & $62.70\pm0.53$& MSD (d=2048) & $66.68\pm0.18$\\ 
 & Basic (d=256) & $64.39\pm0.30$& MSDA (d=16) & $51.57\pm0.39$\\ 
 & Basic (d=512) & $65.95\pm0.19$& MSDA (d=32) & $61.55\pm0.23$\\ 
 & Basic (d=1024) & $66.04\pm0.17$& MSDA (d=64) & $64.94\pm0.50$\\ 
 & Basic (d=2048) & $66.03\pm0.20$& MSDA (d=128) & $66.96\pm0.36$\\ 
 & DSD (d=16) & $49.92\pm0.09$& MSDA (d=256) & $67.63\pm0.34$\\ 
 & DSD (d=32) & $59.75\pm0.78$& MSDA (d=512) & $67.76\pm0.26$\\ 
 & DSD (d=64) & $62.75\pm0.15$& MSDA (d=1024) & $67.79\pm0.10$\\ 
 & DSD (d=128) & $65.57\pm0.26$& MSDA (d=2048) & $67.33\pm0.09$\\ 
 & DSD (d=256) & $66.34\pm0.07$& MSDF (d=16) & $51.99\pm0.57$\\ 
 & DSD (d=512) & $66.89\pm0.15$& MSDF (d=32) & $61.61\pm0.41$\\ 
 & DSD (d=1024) & $66.57\pm0.11$& MSDF (d=64) & $65.31\pm0.23$\\ 
 & DSD (d=2048) & $66.54\pm0.28$& MSDF (d=128) & $66.66\pm0.29$\\ 
 & DSDA (d=16) & $50.77\pm0.71$& MSDF (d=256) & $67.47\pm0.11$\\ 
 & DSDA (d=32) & $60.13\pm0.45$& MSDF (d=512) & $67.59\pm0.03$\\ 
 & DSDA (d=64) & $63.84\pm0.36$& MSDF (d=1024) & $67.40\pm0.15$\\ 
 & DSDA (d=128) & $66.51\pm0.18$& MSDF (d=2048) & $67.01\pm0.35$\\ 
 & DSDA (d=256) & $67.13\pm0.24$& MSDFA (d=16) & $52.96\pm0.44$\\ 
 & DSDA (d=512) & $67.54\pm0.24$& MSDFA (d=32) & $61.98\pm0.36$\\ 
 & DSDA (d=1024) & $67.27\pm0.22$& MSDFA (d=64) & $65.19\pm0.40$\\ 
 & DSDA (d=2048) & $67.33\pm0.30$& MSDFA (d=128) & $67.68\pm0.29$\\ 
 & MSD (d=16) & $50.51\pm0.21$& MSDFA (d=256) & $68.48\pm0.28$\\ 
 & MSD (d=32) & $60.00\pm0.28$& MSDFA (d=512) & $69.06\pm0.14$\\ 
 & MSD (d=64) & $63.74\pm0.24$& MSDFA (d=1024) & $69.08\pm0.22$\\ 
 & MSD (d=128) & $65.80\pm0.16$& MSDFA (d=2048) & $69.29\pm0.35$\\ 
    \bottomrule
    \end{tabular}
    \label{tab:ablations_5}
 \end{table}
 
 
 %%%%%%%%%%%%
 \begin{table}[h]
 \small
   \centering
    \caption{\textit{Experiment: Methods of distillation between reference and target embedding spaces.} See fig. \ref{fig:ablations_1}C. Used Method: \textbf{DSDA}. All results are computed over 5-run averages.}   
   \begin{tabular}{l||c|c}
     \toprule
     Experiment & Setting & R@1\\
     \midrule
\multirow{7}{*}{Distillation Methods} & R-KL & $66.51\pm0.18$\\
 & Cos & $65.73\pm0.27$\\
 & Eucl & $65.61\pm0.28$\\
 & KL-Full & $65.91\pm0.32$\\
 & KL-Mean & $64.00\pm0.55$\\
 & Basic & $62.70\pm0.53$\\
    \bottomrule
    \end{tabular}
    \label{tab:ablations_3}
 \end{table}
 
 
  %%%%%%%%%%%%%%%%
\begin{table}[h]
 \small
   \centering
    \caption{\textit{Experiment: Structure of the secondary branch.} More specifically, this table contains specific values used in fig. \ref{fig:ablations_1}D. Used Method: \textbf{DSDA}. All results are computed over 5-run averages.}   
   \begin{tabular}{l||c|c}
     \toprule
     Experiment & Setting & R@1\\
     \midrule
\multirow{5}{*}{Secondary Branch Structure} & 2 Layers & $66.51\pm0.18$\\
 & 3 Layers & $66.03\pm0.29$\\
 & 4 Layers & $65.76\pm0.65$\\
 & Linear & $65.28\pm0.48$\\
 & Basic & $62.70\pm0.53$\\
    \bottomrule
    \end{tabular}
    \label{tab:ablations_2}
 \end{table}
 

  %%%%%%%
 \begin{table}[h]
 \small
   \centering
    \caption{\textit{Experiment: Different distillation hierarchies.} See fig. \ref{fig:ablations_1}E. Used Method: \textbf{MSDA}. All results are computed over 5-run averages.}   
   \begin{tabular}{l||c|c}
     \toprule
     Experiment & Setting & R@1\\
     \midrule
\multirow{4}{*}{Distillation Hierarchies} & Basic & $62.70\pm0.53$\\
 & Straight & $66.96\pm0.36$\\
 & Fully & $65.58\pm0.46$\\
 & Stacked & $65.21\pm0.25$\\
    \bottomrule
    \end{tabular}
    \label{tab:ablations_10}
 \end{table}
 
 
 %%%%%%%%%%%%%
 \begin{table}[h]
 \small
   \centering
    \caption{\textit{Experiment: Influence of distillation weight $\gamma$.} See fig. \ref{fig:ablations_1}F. Used Method: \textbf{DSD}. All results are computed over 5-run averages.}   
   \begin{tabular}{l||c|c|c|c}
     \toprule
     Experiment & Setting & R@1 CUB200 & R@1 CARS196 & R@1 SOP\\
     \midrule
    \multirow{10}{*}{Weight Ablation} & 0.0 & $62.70\pm0.53$ & $81.32\pm0.36$ & $77.78\pm0.06$\\
     & 0.2 & $62.85\pm0.41$ & $81.65\pm0.40$ & $78.22\pm0.07$\\
     & 1.0 & $62.92\pm0.16$ & $81.92\pm0.51$ & $78.71\pm0.10$\\
     & 5.0 & $63.88\pm0.19$ & $82.96\pm0.10$ & $79.05\pm0.12$\\
     & 20.0 & $65.43\pm0.21$ & $83.50\pm0.35$ & $78.72\pm0.10$\\
     & 50.0 & $65.57\pm0.26$ & $83.51\pm0.33$ & $78.10\pm0.13$\\
     & 250.0 & $65.04\pm0.33$ & $82.25\pm0.62$ & $77.41\pm0.12$\\
     & 1000.0 & $63.32\pm0.36$ & $77.00\pm0.66$ & $77.01\pm0.08$\\
     & 2000.0 & $62.76\pm0.31$ & $72.72\pm0.85$ & $76.37\pm0.11$\\
     & 5000.0 & $62.05\pm0.62$ & $70.90\pm0.97$ & $75.42\pm0.20$\\  

    \bottomrule
    \end{tabular}
    \label{tab:ablations_4}
 \end{table}



 
 %%%%%%%
 \begin{table}[h]
 \small
   \centering
    \caption{\textit{Experiment: Evaluation target dimensions and levels of multiscale distillation.} See fig. \ref{fig:ablations_2}A. All results are computed over 5-run averages.}   
   \begin{tabular}{l||c|c}
     \toprule
     Experiment & Setting & R@1\\
     \midrule
\multirow{5}{*}{Target Dimensionalities} & Basic & $62.70\pm0.53$\\
 & DSDA, TD=256 & $64.82\pm0.18$\\
 & DSDA, TD=512 & $66.44\pm0.31$\\
 & DSDA, TD=1024 & $66.25\pm0.26$\\
 & DSDA, TD=2048 & $66.51\pm0.18$\\
\multirow{4}{*}{MultiScale distillation} & MSDA, \#B=2 & $66.76\pm0.23$\\
 & MSDA, \#B=4 & $66.96\pm0.36$\\
 & MSDA, \#B=8 & $66.72\pm0.25$\\
 & MSDA, \#B=16 & $66.59\pm0.20$\\
    \bottomrule
    \end{tabular}
    \label{tab:ablations_7}
 \end{table}



%%%%%%%%
 \begin{table}[h]
 \small
   \centering
    \caption{\textit{Experiment: Is it beneficial to distill more fine-grained features?} See fig. \ref{fig:ablations_2}B. All results are computed over 5-run averages.}
    \label{tab:ablations_8}   
   \begin{tabular}{l||c|c}
     \toprule
     Experiment & Setting & R@1\\
     \midrule
\multirow{7}{*}{Earlier Features} & Basic & $62.70\pm0.53$\\
 & MSDA & $66.96\pm0.36$\\
 & MSDFA & $67.68\pm0.29$\\
 & MSDFA, \#P=1 & $66.13\pm0.22$\\
 & MSDFA, \#P=2 & $65.49\pm0.12$\\
 & MSDFA, \#P=3 & $66.22\pm0.24$\\
 & MSDFA, \#P=4 & $65.96\pm0.04$\\
    \bottomrule
    \end{tabular}
 \end{table}
 
 
 %%%%%%%
 \begin{table}[h]
 \small
   \centering
    \caption{\textit{Experiment: Is it necessary to detach auxiliary branches for distillation?} See fig. \ref{fig:ablations_2}C. All results are computed over 5-run averages.}   
   \begin{tabular}{l||c|c}
     \toprule
     Experiment & Setting & R@1\\
     \midrule
\multirow{5}{*}{Branch Detaching} & Basic & $62.70\pm0.53$\\
 & DSDA, Detached & $66.51\pm0.18$\\
 & DSDA, Non-Detach & $65.08\pm0.23$\\
 & MSDA, Detached & $66.96\pm0.36$\\
 & MSDA, No-Detach & $65.34\pm0.07$\\
    \bottomrule
    \end{tabular}
    \label{tab:ablations_9}
 \end{table}

  

   


==> tables/old_sota.tex <==
\begin{table*}[t]
    \caption{\textit{State-of-the-art comparison.} We show that our self-distillation module (\textit{SMSD}) achieves state-of-the-art across literature. ($^*$) stands for IBN with frozen Batch-Norm, ($^\dagger$) notes global max- \& average pooling throughout \cite{kim2020proxy}. ($^+$) means larger images used.}
    \setlength\tabcolsep{1.5pt}
    \footnotesize
    \centering
    \resizebox{\textwidth}{!}{
     \begin{tabular}{l||c|c|c||c|c|c||c|c|c}
         \toprule
         Benchmark $\rightarrow$ & \multicolumn{3}{c}{CUB200-2011} & \multicolumn{3}{c}{CARS196}& \multicolumn{3}{c}{SOP}\\
         \midrule
         Approach $\downarrow$ & R@1 & R@2 & NMI & R@1 & R@2 & NMI & R@1 & R@10 & NMI \\
         \midrule
         \hline
         \multicolumn{10}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-128}} \\
         \hline
         \rowcolor{vvlightgray}
         D\&C \cite{Sanakoyeu_2019_CVPR}  & 65.9 & 76.6 & 69.6 & 84.6 & 90.7 & 70.3 & 75.9 & 88.4 & 90.2\\
         \rowcolor{vvlightgray}
         MIC \cite{mic}                   & 66.1 & 76.8 & 69.7 & 82.6 & 89.1 & 68.4 & 77.2 & 89.4 & 90.0\\
         \rowcolor{vvlightgray}
         PADS \cite{roth2020pads}         & 67.3 & 78.0 & 69.9 & 83.5 & 89.7 & 68.8 & 76.5 & 89.0 & 89.9\\
         \hline
         Multisimilarity+\textit{SMSD}     & 68.0  $\pm$  0.2 & 78.7 $\pm$ 0.1 & 71.7 $\pm$ 0.4 & 86.3 $\pm$ 0.1 & 91.8 $\pm$ 0.3 & 72.0 $\pm$ 0.3 & 79.0 $\pm$ 0.2 & 90.2 $\pm$ 0.1 & 90.6 $\pm$ 0.1\\
         Margin+\textit{SMSD}            & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & 80.2 $\pm$ 0.2 & 91.5 $\pm$ 0.1 & 90.9 $\pm$ 0.1\\
         R-Margin+\textit{SMSD}          & \textbf{68.9}  $\pm$  \textbf{0.3} & \textbf{79.0} $\pm$ \textbf{0.3} & \textbf{72.1} $\pm$ \textbf{0.4} & \textbf{87.6} $\pm$ \textbf{0.2} & \textbf{92.7} $\pm$ \textbf{0.2} & \textbf{72.3} $\pm$ \textbf{0.2} & 79.2 $\pm$ 0.2 & 90.3 $\pm$ 0.1 & 90.8 $\pm$ 0.1\\
         \midrule
         \hline
         \multicolumn{10}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-512}} \\
         \hline
         \rowcolor{vvlightgray}
         DiVA \cite{milbich2020diva}   & 69.2 & 79.3 & 71.4 & 87.6 & 92.9 & 72.2 & 79.6 & 91.2 & 90.6\\
         \hline
         Multisimilarity+\textit{SMSD}  & 69.2 $\pm$ 0.1 & 79.1 $\pm$ 0.2 & 71.4 $\pm$ 0.2 & 89.1 $\pm$ 0.2 & 93.8 $\pm$ 0.2 & 74.0 $\pm$ 0.2 & - & - & -\\
         Margin+\textit{SMSD}           & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
         R-Margin+\textit{SMSD}         & 69.7 $\pm$ 0.2 & 79.5 $\pm$ 0.3 & 71.6 $\pm$ 0.2 & 89.5 $\pm$ 0.2 & 93.8 $\pm$ 0.3 & 72.9 $\pm$ 0.3 & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
         % \red{N} DiVA+\textit{SMSD}     & - & - & - & - & - & - & - & - & -\\
         \midrule
         \hline
         \multicolumn{10}{>{\columncolor[gray]{.8}}l}{\textbf{Inception-BN-512}} \\
         \hline
         \rowcolor{vvlightgray}
         HORDE$^+$ \cite{horde}         & 66.3 & 76.7 & -      & 83.9 & 90.3 & -      & 80.1      & 91.3      & -     \\
         \rowcolor{vvlightgray}
         DiVA \cite{milbich2020diva}    & 66.8 & 77.7 & 70.0 & 84.1 & 90.7 & 68.7 & 78.1 & 90.6 & 90.4\\
         \hline
         Multisimilarity+\textit{SMSD}   & 66.6 $\pm$ 0.3 & 77.5 $\pm$ 0.3 & 70.5 $\pm$ 0.2 & 83.6 $\pm$ 0.3 & 90.3 $\pm$ 0.2 & 69.8 $\pm$ 0.3 & 78.5 $\pm$ 0.2 & 90.6 $\pm$ 0.2 & 90.6 $\pm$ 0.1\\
         Margin+\textit{SMSD}            & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
         R-Margin+\textit{SMSD}          & 67.4 $\pm$ 0.3 & 78.0 $\pm$ 0.4 & 70.3 $\pm$ 0.2 & 83.8 $\pm$ 0.3 & 90.3 $\pm$ 0.2 & 69.4 $\pm$ 0.2 & - & - & -\\
         \hline
         \rowcolor{vvlightgray}
         Softtriple$^*$ \cite{softriple}              & 65.4 & 76.4 & -      & 84.5 & 90.7 & 70.1 & 78.3 & 90.3 & 92.0\\
         \rowcolor{vvlightgray}
         Multisimilarity$^*$ \cite{multisimilarity}   & 65.7 & 77.0 & -      & 84.1 & 90.4 & -      & 78.2 & 90.5 & -     \\
         \hline
         Multisimilarity$^*$+\textit{SMSD}             & 68.2 $\pm$ 0.3 & 79.1 $\pm$ 0.2 & 71.6 $\pm$ 0.2 & 86.3 $\pm$ 0.2 & 92.2 $\pm$ 0.2 & 72.0 $\pm$ 0.3 & 78.9 $\pm$ 0.2 & - $\pm$ - & 90.6 $\pm$ 0.1\\
         Margin$^*$+\textit{SMSD}                      & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
         R-Margin$^*$+\textit{SMSD}                    & 69.6 $\pm$ 0.3 & 79.7 $\pm$ 0.3 & 71.2 $\pm$ 0.1 & 86.6 $\pm$ 0.3 & 92.1 $\pm$ 0.3 & 70.9 $\pm$ 0.2 & - & - & -\\
         \hline
         \rowcolor{vvlightgray}
         ProxyAnchor$^{*\dagger}$ \cite{kim2020proxy}   & 68.4  & 79.2       & -            & 86.1 & 91.7 & -    & 79.1 & 90.8 & -\\
         \hline
         Multisimilarity$^{*\dagger}$+\textit{SMSD}      & 69.0 $\pm$ 0.2 & 79.5 $\pm$ 0.2 & 71.7 $\pm$ 0.2 & 87.8 $\pm$ 0.2 & 93.1 $\pm$ 0.2 & 73.3 $\pm$ 0.3 & & &\\
         Margin$^{*\dagger}$+\textit{SMSD}               & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
         ProxyAnchor$^{*\dagger}$+\textit{SMSD}          & 69.5 $\pm$ 0.2 & 79.8 $\pm$ 0.2 & 71.3 $\pm$ 0.2 & 87.2 $\pm$ 0.3 & 92.6 $\pm$ 0.2 & 70.5 $\pm$ 0.4 & - & - & -\\
         % DiVA+\textit{SMSD}                & 70.1 $\pm$ 0.2 & 80.1 $\pm$ 0.2 & 72.5 $\pm$ 0.3 & - & - & - & - & - & -\\
         \bottomrule
    \end{tabular}}
    \label{tab:sota}
\end{table*}


==> tables/slighly_old_sota.tex <==



\begin{table*}[t]
    \caption{\textit{State-of-the-art comparison.} We show that our self-distillation module (\textit{SMSD}) achieves state-of-the-art across literature. ($^*$) stands for IBN with frozen Batch-Norm, ($^\dagger$) notes global max- \& average pooling throughout \citep{kim2020proxy}.}% ($^+$) means larger images used.}
    \setlength\tabcolsep{1.5pt}
    \footnotesize
    \centering

\resizebox{\textwidth}{!}{
 
 \begin{tabular}{l||c|c|c}
     \toprule
     Benchmark $\rightarrow$ & \multicolumn{3}{c}{CUB200 \citep{cub200-2011}}\\
     \midrule
     Approach $\downarrow$ & R@1 & R@2 & NMI\\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-128}} \\
     \hline
     \rowcolor{vvlightgray}
     Div\&Conq \citep{Sanakoyeu_2019_CVPR}  & 65.9 & 76.6 & 69.6\\
     \rowcolor{vvlightgray}
     MIC \citep{mic}                   & 66.1 & 76.8 & 69.7\\
     \rowcolor{vvlightgray}
     PADS \citep{roth2020pads}         & 67.3 & 78.0 & 69.9\\
     \hline
     Multisimilarity+\textit{SMSD}     & 68.0  $\pm$  0.2 & 78.7 $\pm$ 0.1 & 71.7 $\pm$ 0.4 \\
     Margin+\textit{SMSD}      & 67.6  $\pm$  0.3 & 78.2 $\pm$ 0.2 & 70.8 $\pm$ 0.3 \\
     R-Margin+\textit{SMSD}    & \textbf{68.9}  $\pm$  \textbf{0.3} & \textbf{79.0} $\pm$ \textbf{0.3} & \textbf{72.1} $\pm$ \textbf{0.4} \\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-512}} \\
     \hline
     \rowcolor{vvlightgray}
     EPSHN \citep{epshn}                     & 64.9 & 75.3 &  -   \\
     \rowcolor{vvlightgray}
     NormSoft \citep{zhai2018classification} & 61.3 & 73.9 &  -   \\
     \rowcolor{vvlightgray}
     DiVA \citep{milbich2020diva}            & 69.2 & 79.3 & 71.4 \\
     \hline
     Multisimilarity+\textit{SMSD}  & 69.2 $\pm$ 0.1 & 79.1 $\pm$ 0.2 & 71.4 $\pm$ 0.2 \\
     Margin+\textit{SMSD}           & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
     R-Margin+\textit{SMSD}         & 69.7 $\pm$ 0.2 & 79.5 $\pm$ 0.3 & 71.6 $\pm$ 0.2 \\
     % \red{N} DiVA+\textit{SMSD}     & - & - & - \\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{Inception-BN-512}} \\
     \hline
    %  \rowcolor{vvlightgray}
    %  HORDE$^+$          & 66.3 & 76.7 & - \\
     \rowcolor{vvlightgray}
     DiVA \citep{milbich2020diva}    & 66.8 & 77.7 & 70.0 \\
     \hline
     Multisimilarity+\textit{SMSD}   & 66.6 $\pm$ 0.3 & 77.5 $\pm$ 0.3 & 70.5 $\pm$ 0.2 \\
     Margin+\textit{SMSD}            & 66.8 $\pm$ 0.2 & 77.9 $\pm$ 0.2 & 69.9 $\pm$ 0.3 \\
     R-Margin+\textit{SMSD}          & 67.4 $\pm$ 0.3 & 78.0 $\pm$ 0.4 & 70.3 $\pm$ 0.2 \\
     \hline
     \rowcolor{vvlightgray}
     Softtriple$^*$ \citep{softriple} & 65.4 & 76.4 & -  \\
     \rowcolor{vvlightgray}
     Multisimilarity$^*$ \citep{multisimilarity} & 65.7 & 77.0 & -  \\
     \hline
     Multisimilarity$^*$+\textit{SMSD}             & 68.2 $\pm$ 0.3 & 79.1 $\pm$ 0.2 & 71.6 $\pm$ 0.2 \\
     Margin$^*$+\textit{SMSD}                      & 68.3 $\pm$ 0.2 & 78.8 $\pm$ 0.2 & 71.2 $\pm$ 0.2 \\
     R-Margin$^*$+\textit{SMSD}                    & 69.6 $\pm$ 0.3 & 79.7 $\pm$ 0.3 & 71.2 $\pm$ 0.1 \\
     \hline
     \rowcolor{vvlightgray}
     ProxyAnchor$^{*\dagger}$ \citep{kim2020proxy} & 68.4  & 79.2       & -           \\
     \hline
     Multisimilarity$^{*\dagger}$+\textit{SMSD}      & 69.0 $\pm$ 0.2 & 79.5 $\pm$ 0.2 & 71.7 $\pm$ 0.2 \\
     Margin$^{*\dagger}$+\textit{SMSD}               & 68.3 $\pm$ 0.3 & 78.4 $\pm$ 0.3 & 70.4 $\pm$ 0.2 \\
     ProxyAnchor$^{*\dagger}$+\textit{SMSD}          & 69.5 $\pm$ 0.2 & 79.8 $\pm$ 0.2 & 71.3 $\pm$ 0.2 \\
     % DiVA+\textit{SMSD}                & 70.1 $\pm$ 0.2 & 80.1 $\pm$ 0.2 & 72.5 $\pm$ 0.3 \\
     \bottomrule
\end{tabular}

 \begin{tabular}{l||c|c|c}
     \toprule
     Benchmark $\rightarrow$ & \multicolumn{3}{c}{CARS196 \citep{cars196}}\\
     \midrule
     Approach $\downarrow$ & R@1 & R@2 & NMI \\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-128}} \\
     \hline
     \rowcolor{vvlightgray}
     Div\&Conq \citep{Sanakoyeu_2019_CVPR} & 84.6 & 90.7 & 70.3\\
     \rowcolor{vvlightgray}
     MIC \citep{mic}               & 82.6 & 89.1 & 68.4\\
     \rowcolor{vvlightgray}
     PADS \citep{roth2020pads}     & 83.5 & 89.7 & 68.8\\
     \hline
     Multisimilarity+\textit{SMSD}   & 86.3 $\pm$ 0.1 & 91.8 $\pm$ 0.3 & 72.0 $\pm$ 0.3\\
     Margin+\textit{SMSD}    & 86.0 $\pm$ 0.2 & 91.8 $\pm$ 0.2 & 72.2 $\pm$ 0.2 \\
     R-Margin+\textit{SMSD}  & \textbf{87.6} $\pm$ \textbf{0.2} & \textbf{92.7} $\pm$ \textbf{0.2} & \textbf{72.3} $\pm$ \textbf{0.2}\\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-512}} \\
     \hline
     \rowcolor{vvlightgray}
     EPSHN \citep{epshn}                     & 82.7 & 89.3 &  -   \\
     \rowcolor{vvlightgray}
     NormSoft \citep{zhai2018classification} & 84.2 & 90.4 &  - \\     
     \rowcolor{vvlightgray}
     DiVA \citep{milbich2020diva}            & 87.6 & 92.9 & 72.2\\
     \hline
     Multisimilarity+\textit{SMSD}    & 89.1 $\pm$ 0.2 & 93.8 $\pm$ 0.2 & 74.0 $\pm$ 0.2\\
     Margin+\textit{SMSD}     & - $\pm$ - & - $\pm$ - & - $\pm$ - \\
     R-Margin+\textit{SMSD}   & 89.5 $\pm$ 0.2 & 93.8 $\pm$ 0.3 & 72.9 $\pm$ 0.3 \\
     % \red{N} DiVA+\textit{SMSD}   & - & - & - \\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{Inception-BN-512}} \\
     \hline
    %  \rowcolor{vvlightgray}
    %  HORDE$^+$         & 83.9 & 90.3 & - \\
     \rowcolor{vvlightgray}
     DiVA \citep{milbich2020diva}   & 84.1 & 90.7 & 68.7\\
     \hline
     Multisimilarity+\textit{SMSD}   & 83.6 $\pm$ 0.3 & 90.3 $\pm$ 0.2 & 69.8 $\pm$ 0.3\\
     Margin+\textit{SMSD}            & 84.1 $\pm$ 0.2 & 90.6 $\pm$ 0.2 & 69.8 $\pm$ 0.2 \\
     R-Margin+\textit{SMSD}          & 83.8 $\pm$ 0.3 & 90.3 $\pm$ 0.2 & 69.4 $\pm$ 0.2\\
     \hline
     \rowcolor{vvlightgray}
     Softtriple$^*$ \citep{softriple} & 84.5 & 90.7 & 70.1\\
     \rowcolor{vvlightgray}
     Multisimilarity$^*$ \citep{multisimilarity} & 84.1 & 90.4 & -   \\
     \hline
     Multisimilarity$^*$+\textit{SMSD}   & 86.3 $\pm$ 0.2 & 92.2 $\pm$ 0.2 & 72.0 $\pm$ 0.3 \\
     Margin$^*$+\textit{SMSD}            & 87.1 $\pm$ 0.2 & 92.4 $\pm$ 0.1 & 72.2 $\pm$ 0.2 \\
     R-Margin$^*$+\textit{SMSD}          & 86.6 $\pm$ 0.3 & 92.1 $\pm$ 0.3 & 70.9 $\pm$ 0.2\\
     \hline
     \rowcolor{vvlightgray}
     ProxyAnchor$^{*\dagger}$ \citep{kim2020proxy}  & 86.1 & 91.7 & - \\
     \hline
     Multisimilarity$^{*\dagger}$+\textit{SMSD}      & 87.8 $\pm$ 0.2 & 93.1 $\pm$ 0.2 & 73.3 $\pm$ 0.3 \\
     Margin$^{*\dagger}$+\textit{SMSD}               & 87.6 $\pm$ 0.2 & 92.5 $\pm$ 0.2 & 72.6 $\pm$ 0.3 \\
     ProxyAnchor$^{*\dagger}$+\textit{SMSD}          & 87.2 $\pm$ 0.3 & 92.6 $\pm$ 0.2 & 70.5 $\pm$ 0.4\\
     % DiVA+\textit{SMSD}                            & - & - & -\\
     \bottomrule
\end{tabular}}


\resizebox{\textwidth}{!}{
 \begin{tabular}{l||c|c|c}
     \toprule
     Benchmark $\rightarrow$ & \multicolumn{3}{c}{SOP \citep{lifted}} \\
     \midrule
     Approach $\downarrow$ & R@1 & R@10 & NMI \\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-128}} \\
     \hline
     \rowcolor{vvlightgray}
     Div\&Conq \citep{Sanakoyeu_2019_CVPR} & 75.9 & 88.4 & 90.2\\
     \rowcolor{vvlightgray}
     MIC \citep{mic}                  & 77.2 & 89.4 & 90.0\\
     \rowcolor{vvlightgray}
     PADS \citep{roth2020pads}        & 76.5 & 89.0 & 89.9\\
     \hline
     Multisimilarity+\textit{SMSD}     & 79.0 $\pm$ 0.2 & 90.2 $\pm$ 0.1 & 90.6 $\pm$ 0.1\\
     Margin+\textit{SMSD}              & 80.2 $\pm$ 0.2 & 91.5 $\pm$ 0.1 & 90.9 $\pm$ 0.1\\
     R-Margin+\textit{SMSD}            & 79.2 $\pm$ 0.2 & 90.3 $\pm$ 0.1 & 90.8 $\pm$ 0.1\\
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-512}} \\
     \hline
     \rowcolor{vvlightgray}
     EPSHN \citep{epshn}                     & 78.3 & 90.7 &  -   \\
     \rowcolor{vvlightgray}
     NormSoft \citep{zhai2018classification} & 78.2 & 90.6 &  -   \\          
     \rowcolor{vvlightgray}
     DiVA \citep{milbich2020diva}            & 79.6 & 91.2 & 90.6 \\
     \hline
     Multisimilarity+\textit{SMSD}  & 80.8 $\pm$ 0.2 & 92.2 $\pm$ 0.2 & 90.5 $\pm$ 0.3\\
     Margin+\textit{SMSD}           & 81.0 $\pm$ 0.2 & 92.1 $\pm$ 0.2 & 91.1 $\pm$ 0.3\\
     R-Margin+\textit{SMSD}         & 80.0 $\pm$ 0.2 & 91.4 $\pm$ 0.2 & 90.8 $\pm$ 0.1\\
     % \red{N} DiVA+\textit{SMSD}   & - & - & -\\
     \bottomrule
\end{tabular}




 \begin{tabular}{l||c|c|c}
     \toprule
     Benchmark $\rightarrow$ & \multicolumn{3}{c}{SOP \citep{lifted}} \\
     \midrule
     Approach $\downarrow$ & R@1 & R@10 & NMI \\
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{Inception-BN-512}} \\
     \hline
    %  \rowcolor{vvlightgray}
    %  HORDE$^+$         & 80.1      & 91.3      & -     \\
     \rowcolor{vvlightgray}
     DiVA \citep{milbich2020diva}   & 78.1 & 90.6 & 90.4\\
     \hline
     Multisimilarity+\textit{SMSD}   & 78.5 $\pm$ 0.2 & 90.6 $\pm$ 0.2 & 90.6 $\pm$ 0.1\\
     Margin$^*$+\textit{SMSD}        & 78.4 $\pm$ 0.2 & - $\pm$ - & 90.4 $\pm$ 0.1\\
     R-Margin$^*$+\textit{SMSD}      & 78.1 $\pm$ 0.2 & - $\pm$ - & 90.3 $\pm$ 0.2 \\     
     \hline
     \rowcolor{vvlightgray}
     Softtriple$^*$ \citep{softriple} & 78.3 & 90.3 & 92.0\\
     \rowcolor{vvlightgray}
     Multisimilarity$^*$ \citep{multisimilarity}   & 78.2 & 90.5 & -     \\
     \hline
     Multisimilarity$^*$+\textit{SMSD}       & 78.9 $\pm$ 0.2 & - $\pm$ - & 90.6 $\pm$ 0.1\\
     Margin+\textit{SMSD}            & 79.1 $\pm$ 0.2 & - $\pm$ - & 90.4 $\pm$ 0.1\\
     R-Margin+\textit{SMSD}          & 78.5 $\pm$ 0.1 & - $\pm$ - & 90.0 $\pm$ 0.2\\
     \hline
     \rowcolor{vvlightgray}
     ProxyAnchor$^{*\dagger}$ \citep{kim2020proxy}   & 79.1 & 90.8 & -\\
     \hline
     Multisimilarity$^{*\dagger}$+\textit{SMSD} & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
     Margin$^{*\dagger}$+\textit{SMSD}          & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
     ProxyAnchor$^{*\dagger}$+\textit{SMSD}     & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
     % DiVA+\textit{SMSD}                            & - & - & -\\
     \bottomrule
\end{tabular}}


\label{tab:sota}
\end{table*}



==> tables/sota.tex <==


\begin{table*}[t]
    \caption{\textit{State-of-the-art comparison.} We show that \textit{S2SD}, represented by its variants \textit{MSDF(A)}, boosts baseline objectives to state-of-the-art across literature. ($^*$) stands for Inception-V1 with frozen Batch-Norm. \textbf{Bold}: best results per literature setup. \blue{\textbf{Bluebold}}: best results per overall benchmark.}% ($^+$) means larger images used.}
    \setlength\tabcolsep{1.5pt}
    \footnotesize
    \centering

 \begin{tabular}{l||c|c|c||c|c|c||c|c|c}
     \toprule
     Benchmarks $\rightarrow$ & \multicolumn{3}{c||}{CUB200 \cite{cub200-2011}} & \multicolumn{3}{c||}{CARS196 \cite{cars196}} & \multicolumn{3}{c}{SOP \cite{lifted}}\\
     \midrule
     Methods $\downarrow$ & R@1 & R@2 & NMI & R@1 & R@2 & NMI & R@1 & R@10 & NMI\\
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{10}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-128}} \\
     \hline
     \rowcolor{vvlightgray}
     Div\&Conq \cite{Sanakoyeu_2019_CVPR}  & 65.9 & 76.6 & 69.6 & 84.6 & 90.7 & 70.3 & 75.9 & 88.4 & 90.2\\
     \rowcolor{vvlightgray}
     MIC \cite{mic}                        & 66.1 & 76.8 & 69.7 & 82.6 & 89.1 & 68.4 & 77.2 & 89.4 & 90.0\\
     \rowcolor{vvlightgray}
     PADS \cite{roth2020pads}              & 67.3 & 78.0 & 69.9 & 83.5 & 89.7 & 68.8 & 76.5 & 89.0 & 89.9\\
     \hline
     Multisimilarity+\textit{S2SD}         & 68.0  $\pm$  0.2 & 78.7 $\pm$ 0.1 & 71.7 $\pm$ 0.4 & 86.3 $\pm$ 0.1 & 91.8 $\pm$ 0.3 & 72.0 $\pm$ 0.3 & 79.0 $\pm$ 0.2 & 90.2 $\pm$ 0.1 & 90.6 $\pm$ 0.1\\
     Margin+\textit{S2SD}                  & 67.6  $\pm$  0.3 & 78.2 $\pm$ 0.2 & 70.8 $\pm$ 0.3 & 86.0 $\pm$ 0.2 & 91.8 $\pm$ 0.2 & 72.2 $\pm$ 0.2 & \textbf{80.2} $\pm$ \textbf{0.2} & \textbf{91.5} $\pm$ \textbf{0.1} & \textbf{90.9} $\pm$ \textbf{0.1}\\
     R-Margin+\textit{S2SD}                & \textbf{68.9}  $\pm$  \textbf{0.3} & \textbf{79.0} $\pm$ \textbf{0.3} & \textbf{72.1} $\pm$ \textbf{0.4} & \textbf{87.6} $\pm$ \textbf{0.2} & \textbf{92.7} $\pm$ \textbf{0.2} & \textbf{72.3} $\pm$ \textbf{0.2}& 79.2 $\pm$ 0.2 & 90.3 $\pm$ 0.1 & 90.8 $\pm$ 0.1\\
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{10}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-512}} \\
     \hline
     \rowcolor{vvlightgray}
     EPSHN \cite{epshn}                     & 64.9 & 75.3 &  -   & 82.7 & 89.3 &  -  & 78.3 & 90.7 &  -    \\
     \rowcolor{vvlightgray}
     NormSoft \cite{zhai2018classification} & 61.3 & 73.9 &  -   & 84.2 & 90.4 &  -   & 78.2 & 90.6 &  -    \\
     \rowcolor{vvlightgray}
     DiVA \cite{milbich2020diva}            & 69.2 & 79.3 & 71.4 & 87.6 & 92.9 & 72.2 & 79.6 & 91.2 & 90.6 \\
     \hline
     Multisimilarity+\textit{S2SD}          & 69.2 $\pm$ 0.1 & 79.1 $\pm$ 0.2 & 71.4 $\pm$ 0.2 & 89.2 $\pm$ 0.2 & 93.8 $\pm$ 0.2 & \blue{\textbf{74.0} $\pm$ \textbf{0.2}} & 80.8 $\pm$ 0.2 & \blue{\textbf{92.2} $\pm$ \textbf{0.2}} & 90.5 $\pm$ 0.3\\
     Margin+\textit{S2SD}                   & 68.8 $\pm$ 0.2 & 78.5 $\pm$ 0.2 & \blue{\textbf{72.3} $\pm$ \textbf{0.1}} & 89.3 $\pm$ 0.2 & 93.8 $\pm$ 0.2 & 73.7 $\pm$ 0.3 & \blue{\textbf{81.0} $\pm$ \textbf{0.2}} & 92.1 $\pm$ 0.2 & \textbf{91.1} $\pm$ \textbf{0.3}\\
     R-Margin+\textit{S2SD}                 & \blue{\textbf{70.1} $\pm$ \textbf{0.2}} & \blue{\textbf{79.7} $\pm$ \textbf{0.2}} & 71.6 $\pm$ 0.2 & \blue{\textbf{89.5} $\pm$ \textbf{0.2}} & \blue{\textbf{93.9} $\pm$ \textbf{0.3}} & 72.9 $\pm$ 0.3 & 80.0 $\pm$ 0.2 & 91.4 $\pm$ 0.2 & 90.8 $\pm$ 0.1\\
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{10}{>{\columncolor[gray]{.8}}l}{\textbf{Inception-BN-512}} \\
     \hline
    %  \rowcolor{vvlightgray}
    %  HORDE$^+$          & 66.3 & 76.7 & - & \\
     \rowcolor{vvlightgray}
     DiVA \cite{milbich2020diva}     & 66.8 & 77.7 & 70.0 & 84.1 & \textbf{90.7} & 68.7 & 78.1 & \textbf{90.6} & 90.4\\
     \hline
     Multisimilarity+\textit{S2SD}   & 66.7 $\pm$ 0.3 & 77.5 $\pm$ 0.3 & \textbf{70.5} $\pm$ \textbf{0.2} & 83.8 $\pm$ 0.3 & 90.3 $\pm$ 0.2 & \textbf{69.8} $\pm$ \textbf{0.3} & \textbf{78.5} $\pm$ \textbf{0.2} & \textbf{90.6} $\pm$ \textbf{0.2} & \textbf{90.6} $\pm$ \textbf{0.1}\\
     Margin+\textit{S2SD}            & 66.8 $\pm$ 0.2 & 77.9 $\pm$ 0.2 & 69.9 $\pm$ 0.3 & \textbf{84.3} $\pm$ \textbf{0.2} & \textbf{90.7} $\pm$ \textbf{0.2} & \textbf{69.8} $\pm$ \textbf{0.2} & 78.4 $\pm$ 0.2 & 90.5 $\pm$ 0.2 & 90.4 $\pm$ 0.1\\
     R-Margin+\textit{S2SD}          & \textbf{67.4} $\pm$ \textbf{0.3} & \textbf{78.0} $\pm$ \textbf{0.4} & 70.3 $\pm$ 0.2 & 83.9 $\pm$ 0.3 & 90.3 $\pm$ 0.2 & 69.4 $\pm$ 0.2 & 78.1 $\pm$ 0.2 & 90.4 $\pm$ 0.3 & 90.3 $\pm$ 0.2\\
     \hline
     \rowcolor{vvlightgray}
     Softtriple$^*$ \cite{softriple} & 65.4 & 76.4 & 69.3 & 84.5 & 90.7 & 70.1 & 78.3 & 90.3 & \blue{\textbf{92.0}}\\
     \rowcolor{vvlightgray}
     Multisimilarity$^*$ \cite{multisimilarity} & 65.7 & 77.0 & - & 84.1 & 90.4 & -  & 78.2 & 90.5 & -   \\
     \hline
     Multisimilarity$^*$+\textit{S2SD}             & 68.2 $\pm$ 0.3 & 79.1 $\pm$ 0.2 & \textbf{71.6} $\pm$ \textbf{0.2} & 86.3 $\pm$ 0.2 & 92.2 $\pm$ 0.2 & 72.0 $\pm$ 0.3 & 78.9 $\pm$ 0.2 & 90.8 $\pm$ 0.2 & 90.6 $\pm$ 0.1\\
     Margin$^*$+\textit{S2SD}                      & 68.3 $\pm$ 0.2 & 78.8 $\pm$ 0.2 & 71.2 $\pm$ 0.2 & \textbf{87.1} $\pm$ \textbf{0.2} & \textbf{92.4} $\pm$ \textbf{0.1} & \textbf{72.2} $\pm$ \textbf{0.2} & \textbf{79.1} $\pm$ \textbf{0.2} & \textbf{91.0} $\pm$ \textbf{0.3} & 90.4 $\pm$ 0.1\\
     R-Margin$^*$+\textit{S2SD}                    & \textbf{69.6} $\pm$ \textbf{0.3} & \textbf{79.6} $\pm$ \textbf{0.3} & 71.2 $\pm$ 0.1 & 86.6 $\pm$ 0.3 & 92.1 $\pm$ 0.3 & 70.9 $\pm$ 0.2 & 78.5 $\pm$ 0.1 & 90.5 $\pm$ 0.2 & 90.0 $\pm$ 0.2\\
     \bottomrule
\end{tabular}

\label{tab:sota}
\end{table*}



